A flexible scintillation light apparatus for rare event searches

Compelling experimental evidences of neutrino oscillations and their implication that neutrinos are massive particles have given neutrinoless double beta decay a central role in astroparticle physics. In fact, the discovery of this elusive decay would be a major breakthrough, unveiling that neutrino and antineutrino are the same particle and that the lepton number is not conserved. It would also impact our efforts to establish the absolute neutrino mass scale and, ultimately, understand elementary particle interaction unification. All current experimental programs to search for neutrinoless double beta decay are facing with the technical and financial challenge of increasing the experimental mass while maintaining incredibly low levels of spurious background. The new concept described in this paper could be the answer which combines all the features of an ideal experiment: energy resolution, low cost mass scalability, isotope choice flexibility and many powerful handles to make the background negligible. The proposed technology is based on the use of arrays of silicon detectors cooled to 120 K to optimize the collection of the scintillation light emitted by ultra-pure crystals. It is shown that with a 54 kg array of natural CaMoO4 scintillation detectors of this type it is possible to yield a competitive sensitivity on the half-life of the neutrinoless double beta decay of 100Mo as high as ~10E24 years in only one year of data taking. The same array made of 40CaMoO4 scintillation detectors (to get rid of the continuous background coming from the two neutrino double beta decay of 48Ca) will instead be capable of achieving the remarkable sensitivity of ~10E25 years on the half-life of 100Mo neutrinoless double beta decay in only one year of measurement.

==> midef.tex <==
\def\mo100{$^{100}$Mo}
\def\ge76{$^{76}$Ge}
\def\te130{$^{130}$Te}
\def\xe136{$^{136}$Xe}
\def\pb210{$^{210}$Pb}
\def\bi212{$^{212}$Bi}
\def\bi214{$^{214}$Bi}
\def\tl208{$^{208}$Tl}
\def\po212{$^{212}$Po}
\def\po214{$^{214}$Po}
\def\ud238{$^{238}$U}
\def\th232{$^{232}$Th}
\def\camo{CaMoO$_4$}
\def\cdwo{CdWO$_4$}
\def\baf{BaF$_2$}

\def\pbddn{$^{210}$Pb}
\def\podd{$^{210}$Po }
\def\poddn{$^{210}$Po}
\def\udt{$^{238}$U }
\def\udtn{$^{238}$U}
\def\thdt{$^{232}$Th }
\def\thdtn{$^{232}$Th}

\def\tldn{$^{208}$Tl}
\def\bidq{$^{214}$Bi }
\def\bidqn{$^{214}$Bi}
\def\rndd{$^{222}$Rn }
\def\rnddn{$^{222}$Rn}
\def\kq{$^{40}$K }
\def\kqn{$^{40}$K}
\def\coss{$^{60}$Co }
\def\cosn{$^{60}$Co}
\def\pt{$^{190}$Pt }
\def\ptn{$^{190}$Pt}
\def\avl{$\langle \lambda \rangle$~}
\def\ave{$\langle \eta \rangle$~}
\def\avm{$\langle g_{\chi\nu} \rangle$~}
\def\mee{$\langle m_{ee} \rangle$~}
\def\mnu{$\langle m_{\nu} \rangle$~}
\def\amnu{$\vert\langle m_{\nu} \rangle\vert$~}
\def\amnun{$\vert\langle m_{\nu} \rangle\vert$}
\def\nmamnu{\vert\langle m_{\nu} \rangle\vert}
\def\mmod{$\| \langle m_{ee} \rangle \|$}
\def\mb{$\langle m_{\beta} \rangle$~}
\def\fn{$G^{0\nu}\vert M^{0\nu} \vert ^2$}
\def\nmfn{G^{0\nu}\vert M^{0\nu} \vert^2}
\def\BBz{$\beta\beta0\nu$~}
\def\BBzn{$\beta\beta0\nu$}
\def\BBm{$\beta\beta0\nu,\chi$~}
\def\BBd{$\beta\beta(2\nu)$~}
\def\BBdn{$\beta\beta(2\nu)$}
\def\BB{$\beta\beta$~}
\def\Mz{$|M_{0\nu}|$~}
\def\Md{$|M_{2\nu}|$~}
\def\Tz{$T^{0\nu}_{1/2}$~}
\def\Td{$T^{2\nu}_{1/2}$~}
\def\Tm{$T^{0\nu\,\chi}_{1/2}$~}
\def\ca{$\sim$}
\def\dca{$\approx$}
\def\dot{$\cdot$}
\def\pom{$\pm$ }
\def\gm{$\gamma$}
\def\ne{$\neq$}
\def\teod{TeO$_2$~}
\def\teodn{TeO$_2$}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\gohm{G$\Omega$}
\def\ohm{$\Omega$}
\def\per{$\times$}
\def\less{$<$}
\def\gagamma{g_{a\gamma\gamma}}
\def\ciccio{5$\times$5$\times$5 cm$^3$ }
\def\magro{3$\times$3$\times$6 cm$^3$ }
\def\rate{counts/(keV$\cdot$kg$\cdot$y)}

